Atomistic simulations of nanoindentation in single crystalline tungsten: The role of interatomic potentials

Computational modeling is usually applied to aid experimental exploration of advanced materials to better understand the fundamental plasticity mechanisms during mechanical testing. In this work, we perform Molecular dynamics (MD) simulations to emulate experimental room temperature spherical-nanoindentation of crystalline W matrices by different interatomic potentials: EAM, modified EAM, and a recently developed machine learned based tabulated Gaussian approximation potential (tabGAP) for describing the interaction of W-W. Results show similarities between load displacements and stress-strain curves, regardless of the numerical model. However, a discrepancy is observed at early stages of the elastic to plastic deformation transition showing different mechanisms for dislocation nucleation and evolution, that is attributed to the difference of Burgers vector magnitudes, stacking fault and dislocation glide energies. Besides, contact pressure is investigated by considering large indenters sizes that provides a detailed analysis of screw and edge dislocations during loading process. Furthermore, the glide barrier of this kind of dislocations are reported for all the interatomic potentials showing that tabGAP model presents the most accurate results with respect to density functional theory calculations and a good qualitative agreement with reported experimental data

==> sections/uniaxial.tex <==
\section{Uniaxial compression test}
\label{subsec:compression_results}


MD simulations are performed to carry out a uniaxial compression test 
investigating the role of the interatomic potentials in the deformation
mechanisms at room temperature.
We first generate a simulation cell defined by a pillar oriented on $[111]$ 
according to the axis directions defined in Tab. \ref{tab:MD_data}. 
Here, the pillar is defined by 88985 W atoms, a length of 17.78 nm and a 
radius of 5 nm. 
%Larger simulation cell sizes should be used to converge the dislocation nucleation stress 
%values and to not influence the dislocation nucleation mechanism. 
The next step is dedicated to energy optimization of the structure, 
followed by the thermalization to 300 K allowing the lattice constant
to expand to room temperature with a pressure of 0 bar. 
Then, the simulation cell is deformed by a uniaxial strain applied from 0 to 
2\%  on the $z$-direction, that is parallel to the [111] orientation, at a 
strain rate of $5 \times 10^{8}$ s$^{-1}$, while the lateral boundaries
are controlled using the $NPT$ equations of motion 
to zero pressure \cite{WANG201668,GAO2001187} with a time step of 2 fs. 
The [111] orientation is chosen to expect the largest difference 
between stability of nucleated defects.

\begin{figure}[!t]
   \centering
  % \includegraphics[width=0.40\textwidth]{Figures/dislocationNucleation.png}
  \includegraphics[width=0.485\textwidth]{Figures/FigA1.png}
   \caption{(Color on-line). Stress-strain curve of uniaxial compression of 
   a pillar oriented on [111] at room temperature. 
   The simulation cell is deformed by a uniaxial strain applied on the 
   $z$-direction, that is parallel to the [111] orientation, at a strain
   rate of 5 $\times 10^8 s^{-1}$.
   }
   \label{fig:compression}
\end{figure}

MD simulations are performed to investigate the 
mechanical response of W to uniaxial compression test and open boundaries 
by considering plastic deformation of a pillar with a [111] crystal 
orientation. 
In Fig. \ref{fig:compression}, we report results for the stress-strain curve 
at a strain rate of $5\times 10^8$ s$^{-1}$ by every approach considered 
in this work.
During the compression process, the elastic to plastic transition is clearly 
observed by the stress-strain curves with a compression region 
from 0 to 7.5 \% strain for EAM-based potentials, and up to $\sim$ 7 \% 
for EAM with ZBL correction albeit of the curve shape. 
Interstingly, the elastic compression process modeled by modified EAM and 
tabGAP provide similar results, with a different value for the yielding point 
at 13 \% and 15 \%, respectively.
These results show another difference between the approaches used in the 
interatomic potentials parametrization. 
Here, the plastic deformation modeled by tabGAP is quite similar to 
those presented by EAM+ZBL and modified EAM methods. %suggesting that 
%MD simulations performed by tabGAP can lead to a correct interpretation of 
%the results. 



